Learning a Predictable and Generative Vector Representation for Objects

What is a good vector representation of an object? We believe that it should be generative in 3D, in the sense that it can produce new 3D objects; as well as be predictable from 2D, in the sense that it can be perceived from 2D images. We propose a novel architecture, called the TL-embedding network, to learn an embedding space with these properties. The network consists of two components: (a) an autoencoder that ensures the representation is generative; and (b) a convolutional network that ensures the representation is predictable. This enables tackling a number of tasks including voxel prediction from 2D images and 3D model retrieval. Extensive experimental analysis demonstrates the usefulness and versatility of this embedding.

==> conclusion.tex <==
\section{Conclusion}

In this paper, we learn
a predictive and generative embedding space for physical 
objects. We propose a novel TL-embedding network that enables
us to learn such a space by learning an autoencoder over 
3D voxel grids that provides the generative capability, and
a convolutional network that maps RGB to the embedding space.
We perform a series of experiments to analyze the learned manifold,
and show various useful applications such as 3D voxel prediction for
objects and 3D model retrieval, that become possible given this 
representation.

